DRIVE: Dockerfile Rule Mining and Violation Detection

A Dockerfile defines a set of instructions to build Docker images, which can then be instantiated to support containerized applications. Recent studies have revealed a considerable amount of quality issues with Dockerfiles. In this paper, we propose a novel approach DRIVE (Dockerfiles Rule mIning and Violation dEtection) to mine implicit rules and detect potential violations of such rules in Dockerfiles. DRIVE firstly parses Dockerfiles and transforms them to an intermediate representation. It then leverages an efficient sequential pattern mining algorithm to extract potential patterns. With heuristic-based reduction and moderate human intervention, potential rules are identified, which can then be utilized to detect potential violations of Dockerfiles. DRIVE identifies 34 semantic rules and 19 syntactic rules including 9 new semantic rules which have not been reported elsewhere. Extensive experiments on real-world Dockerfiles demonstrate the efficacy of our approach.

==> sections/validity.tex <==
{\color{red}\section{Threats to Validity}\label{validity}}
{\color{red}\subsection{Construct validity} This aspect of validity is related with the degree to which variables represent the concepts~\cite{sjoberg2022}. In our approach, we solely rely on the sequence patterns mined from the Dockerfiles to extract potential rules. To balance the efficiency and accuracy, we leverage a set of heuristics and abstraction rules to accelerate the mining process. These heuristics are based on domain experts and observations. To mitigate the potential errors introduced in this process, we double check these heuristics and hire human experts to manually check the selected samples after processing. For the detection part of \toolname, we use the typical measurements to evaluate the performance, such as precision, recall, and F-measure, which are widely used in the literature.}
{\color{red}\subsection{Internal validity} The threats arising from this aspect are mainly introduced from the bias of the collected data in our approach. To mitigate this, we collect an initial Dockerfile dataset from a diversity of domains and programming languages. Then we select projects with high star numbers as the initial data source. This metric is a direct indicator for popularity~\cite{borges2016} and widely used as a criterion to select GitHub projects in empirical studies in software engineering~\cite{borges2018}. More popular projects attract more attention and more participation which are crucial for open source software quality assurance. Therefore, indirectly, projects with more stars are more likely to be of higher quality. To be more rigorous, we set 1000 stars, which is indeed a high number, as the threshold for the initial filtering. In the remaining projects, we use a set of heuristics, including both tool support and human examination, to further select high quality Dockerfiles. The selection criteria are based on the public tags and commonly used in similar research practice.}
{\color{red}\subsection{External validity} The external validity is  mainly about the generalization issues of the proposed approach. We admit that in our approach, it is impractical to collect all the high quality Dockerfiles based on which all rules could be automatically extracted. However, we demonstrated that with the current collected data, our approach could already find many interesting rules, some of which have not been covered in the state-of-the-art tools. On the other hand, the methodology of our approach, i.e., applying data mining techniques to other software artifacts to find potential patterns, has also well been demonstrated by related work in the literature~\cite{bian2018nar,li2005pr,liang2016antminer}.}
